Bandpass mismatch error for satellite CMB experiments II: Correcting for the spurious signal

Future Cosmic Microwave Background (CMB) satellite missions aim at using the B-mode polarisation signal to measure the tensor-to-scalar ratio $r$ with a sensitivity $\sigma(r)$ of the order of $\leq 10^{-3}$. Small uncertainties in the characterisation of instrument properties such as the spectral filters can lead to a leakage of the intensity signal to polarisation and can possibly bias any measurement of a primordial signal. In this paper we discuss methods for avoiding and correcting for the intensity to polarisation leakage due to bandpass mismatch among detector sets. We develop a template fitting map-maker to obtain an unbiased estimate of the leakage signal and subtract it out of the total signal. Using simulations we show how such a method can reduce the bias on the observed B-mode signal by up to $3$ orders of magnitude in power.

==> sec-abstract.tex <==
\abstract{Future Cosmic Microwave Background (CMB) satellite missions aim to use the B-mode polarisation signal to measure the tensor-to-scalar ratio $r$ with a sensitivity of the order of $\sigma(r)\leq 10\pow{-3}$. Small uncertainties in the characterisation of instrument properties such as the spectral filters will lead to a leakage of the intensity signal to polarisation and possibly mask any primordial signal. In this paper we discuss methods for avoiding and correcting for the intensity to polarisation leakage due to bandpass mismatch among detector sets. We develop a template fitting map-maker to obtain an unbiased estimate of the leakage signal. Using simulations we show how such a method can reduce the bias on the observed B-mode signal by up to $3$ orders of magnitude in power.}


